V3D-SLAM: Robust RGB-D SLAM in Dynamic Environments with 3D Semantic Geometry Voting

Simultaneous localization and mapping (SLAM) in highly dynamic environments is challenging due to the correlation complexity between moving objects and the camera pose. Many methods have been proposed to deal with this problem; however, the moving properties of dynamic objects with a moving camera remain unclear. Therefore, to improve SLAM's performance, minimizing disruptive events of moving objects with a physical understanding of 3D shapes and dynamics of objects is needed. In this paper, we propose a robust method, V3D-SLAM, to remove moving objects via two lightweight re-evaluation stages, including identifying potentially moving and static objects using a spatial-reasoned Hough voting mechanism and refining static objects by detecting dynamic noise caused by intra-object motions using Chamfer distances as similarity measurements. Our experiment on the TUM RGB-D benchmark on dynamic sequences with ground-truth camera trajectories showed that our methods outperform the most recent state-of-the-art SLAM methods. Our source code is available at https://github.com/tuantdang/v3d-slam.

==> notes.tex <==

% \textbf{Methods}:
% \begin{enumerate}
%     \item Estimate pose between two frames using two sensing modalities: RGB-D and LIDAR. LIDAR is used to estimate precise pose in 3D, and RGB-D is used to capture rich data from the environment for downstream tasks like fine-grained object detection.
%     \item Alignment technique between RGB-D and LIDAR is presented by searching the same object in data presentation from RGB-D and LIDAR.
%     \item Real-time pose estimation is performed in a small embedded computer, which calculates the rotation and translation between two poses from 3D  corresponding key points. The corresponding key points are estimated from RGB images and then refined by LIDAR data to remove the wrong pair due to the error in estimation under a variant of lighting and camera pose.
% \end{enumerate}

% Challenges: both robot and tracked objects are moving. Robot relies on its odometry to track the change of posing.

% T1 sampling: 

% \begin{itemize}
%     \item Mapping building and science construction at the same time
%     \item Scence understanding 
%     \item Previous works reconstruct a scene from a single frame
%     \item Previous 3Dmapping focus only on layout on horizontal and verticle, ignoring the objects in the science. It amain for navigation tasks, but task is getting more complex if manipulation is involved
%     \item Sampling from geometry prime shape with sensor models? $sample(Shape, SensorType)$
    
%     \item Maintain parallelism attracts lightweight (obstible avoidance, nagvigation) and detailed map (manupluation) at the same time for different purposes. 
%     \item Estimate pose changes using LIDAR : using sampling from simple 3D geometric with sensor model
%     \item Construct Map using Voxblox knowing camera pose
% \end{itemize}

% \begin{itemize}
%     \item Simple test rotate RGB-D camamera and registrate them into single PC than analy them.
%     \item 3D map representation? 3D occupancy ? why not? point cloud ? why not? Graph more efficient and how to ap transform from RGB-D to Graph based representation?
% \end{itemize}

% Limitation of previous works
% \begin{itemize}
%     \item Detect or Segment 2D then reconstruct 3D scene by depth information obtained from RGB-D camera: (1) light condition/occlusion/object in object, (2) slow since dense RGB will be computed on entire image.
%     \item Voxel representation is subjected to quantilizatin or descreterize 
% \end{itemize}

